Optical Cross-Match of SRG/eROSITA X-ray Sources Using the Deep Lockman Hole Survey as an Example

We present a method for the optical identification of sources detected in wide-field X-ray sky surveys. We have constructed and trained a neural network model to characterise the photometric attributes of the populations of optical counterparts of X-ray sources and optical field objects. The photometric information processing result is used for the probabilistic cross-match of X-ray sources with optical DESI Legacy Imaging Surveys sources. The efficiency of the method is illustrated using the SRG/eROSITA Survey of Lockman Hole. To estimate the accuracy of the method, we have produced a validation sample based on the Chandra and XMM-Newton catalogues of X-ray sources. The cross-match precision in our method reaches 94% for the entire X-ray catalogue and 97% for sources with a flux $F_{\rm x, 0.5-2}>10^{-14}$ erg/s/cm$^2$. We discuss the further development of the optical identification model and the steps needed for its application to the SRG/eROSITA all-sky survey data.

==> figures/nnmag_table.tex <==
\begin{tabular}{c|cccc}
Model         & Features                                                                                & Sample size$^1$                                               & Network structure                                                                    & Overall quality$^2$ \\\hline\hline
nnmag\_grzw1w2 & \begin{tabular}[c]{@{}c@{}}g,r,z, w1, w2\\ g-r,r-z,g-z\\ z-w1, r-w1, w1-w2\end{tabular} & \begin{tabular}[c]{@{}c@{}}1: 10480\\ 0: 55636\end{tabular}  & \begin{tabular}[c]{@{}c@{}}4 layers with 8 neurons\\ Dropout rate: 0.1\end{tabular}  & 0.67           \\\hline
nnmag\_grzw1   & \begin{tabular}[c]{@{}c@{}}g,r,z, w1\\ g-r,r-z,g-z, z-w1\end{tabular}                     & \begin{tabular}[c]{@{}c@{}}1: 10814\\ 0: 89670\end{tabular}  & \begin{tabular}[c]{@{}c@{}}4 layers with 8 neurons\\ Dropout rate: 0.1\end{tabular}  & 0.61           \\\hline
nnmag\_grz     & \begin{tabular}[c]{@{}c@{}}g,r,z\\ g-r,r-z,g-z\end{tabular}                             & \begin{tabular}[c]{@{}c@{}}1: 11092\\ 0: 141845\end{tabular} & \begin{tabular}[c]{@{}c@{}}2 layers with 13 neurons\\ Dropout rate: 0.0\end{tabular} & 0.38      
\end{tabular}

==> figures/quality_table.tex <==

\begin{tabular}{c|cccccc}
Model                                                                                          & \begin{tabular}[c]{@{}c@{}}Companion\\ is correct\\ (A)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Companion\\ is incorrect\\ (B)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Companion \\ assigned\\ to hostless\\ (C)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Source \\ with companion\\ assigned hostless\\ (D)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Correct\\ hostless\\ (E)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Model \\ quality\end{tabular} \\ \hline
\begin{tabular}[c]{@{}c@{}}NWAY + \\ nnmag\\ $p_{\rm any, 0} = 0.12$\end{tabular}                   & 503                                                              & 20                                                                 & 6                                                                                    & 6                                                                                               & 24                                                              & Q = 0.94                                                   \\ \hline
\begin{tabular}[c]{@{}c@{}}closest\\ candidate\\ $p_{\rm any, 0} = 0.24$\end{tabular}               & 460                                                              & 61                                                                 & 9                                                                                   & 8                                                                                               & 21                                                              & Q = 0.86                                                   \\ \hline
\begin{tabular}[c]{@{}c@{}}NWAY + \\ nnmag\\ (bright sources)\\ $p_{\rm any, 0} = 0.11$\end{tabular} & 246                                                              & 4                                                                  & 0                                                                                    & 0                                                                                               & 3                                                               & Q = 0.98                                                   \\ \hline
\end{tabular}

